Exploring Superconductivity: The Interplay of Electronic Orders in Topological Quantum Materials

Topological quantum materials hold great promise for future technological applications. Their unique electronic properties, such as protected surface states and exotic quasiparticles, offer opportunities for designing novel electronic devices, spintronics, and quantum information processing. The origin of the interplay between various electronic orders in topological quantum materials, such as superconductivity and magnetism, remains unclear, particularly whether these electronic orders cooperate, compete, or simply coexist. Since the 2000s, the combination of topology and matter has sparked a tremendous surge of interest among theoreticians and experimentalists alike. Novel theoretical descriptions and predictions, as well as complex experimental setups confirming or refuting these theories, continuously appear in renowned journals. This review aims to provide conceptual tools to understand the fundamental concepts of this ever-growing field. Superconductivity and its historical development will serve as a second pillar alongside topological materials. While the primary focus will be on topological superconductors, other topological materials, such as topological insulators and topological semimetals, will also be explained phenomenologically.

==> 2_Fundamentals.tex <==




==> notused.tex <==
Models for this rather new class of materials existed, such as the Hubbard model, but it was not until Metzner and Vollhardt introduced dimensions (degrees of freedom for a given electron) $d\rightarrow \infty$, so that the equation of motions could be solved, which also solved impurity problems of the system \cite{MetznerVollhardt1989}. Using Methner and Vollhardt's approach, a Dynamical Mean-Field Theory was developed, which enabled physicists to model electrons being only dependent on energy and time, but not dependent on the spatial wave vector. 

SC gap:

The principle of STMs is very straightforward: One uses a metallic tip (if interested in magnetic behaviour, one may use a ferromagnetic tip) and places the tip a few Ångströms above the surface. Quantum mechanical tunnelling from the surface to the tip occurs, resulting in a tunnelling current. The STM then scans across the surface and keeps track of currents at all positions to create a map, keeping the distance to the surface steady via an electronic feedback loop. Clearly this technique is unsuitable for bulk measurements\cite{fischer2007scanning}. To acquire measurements on the superconducting gap, one needs to measure $dI/dV$ dependence (the conductance), as shown in figure \ref{conductctance}.

The  peak, often referred to as the Zero-bias conductance peak (ZBCP) is caused by the Andreev reflection mechanism between a normal-state (NS) material and a SC\cite{pannetier2000andreev}. As might be expected, the electrical current changes, when entering a SC from a NS material as conditions in the material change entirely into loss-free electron transport\cite{pannetier2000andreev}\cite{andreev1964thermal}\cite{ko2022noncontact}. When a small voltage is applied ($eV$ typically lower than $\Delta$), the energy of the electron is too small to enter the SC, thus the electron is reflected. However, two reflections are possible: normal reflection and Andreev reflection. Andreev reflection implies that upon the arrival of the electron at the interface, a hole is created and reflected back into the NS material, while a Cooper pair may form in the SC. In terms of the differential $I-V$ diagram, as shown in figure \ref{conductctance} a), this gives rise to the probabililty amplitude of an electron being transmitted through the junction\cite{narlikar2017oxford}.

In figure \ref{conductctance} a), a typical conductance spectrum of varying thin film thicknesses and temperatures is shown. The magnitude of the ZBC peak thus not only depends on temperature, which has been well-established for bulk SCs\cite{poole2013superconductivity}, but also layer thickness. The normalized conductance is the conductivity at certain low temperatures (as displayed in the figure) divided by normal-state (non-superconducting) conductivity at a much higher temperature (for example: 350 K). These peaks and their magnitudes may then be fitted with BCS theory to yield the experimental phase transition diagram\cite{bardeen1957theory}, displayed in figure \ref{conductctance} b). One may then also use the acquired data to approximate $\Delta_{0}$, the superconducting gap at $T=0K$\cite{eom2006persistent}. To show the layer dependence of $\Delta$ more clearly, Eom et al. took the ZBC peaks of figure \ref{conductctance} a) and plotted them for three temperatures in figure \ref{conductctance} c).

\begin{figure}
    \centering
    \captionsetup{justification=centering}
    \includegraphics[width=0.7\textwidth]{superconducting gap.jpg}
    \caption{Extraction of superconducting gaps for different numbers of layers (5, 6 and 7) of $Pb$. \newline a) Normalized conductance vs. bias voltage ($dI/dV$) at different temperatures for different layer thicknesses b) BCS-like superconducting gaps and predicted behaviour (solid lines) c) Zero bias conductance peaks at different temperatures. Taken from \cite{eom2006persistent}.}
    \label{conductctance}
\end{figure}









